Context-Aware Streaming Perception in Dynamic Environments

Efficient vision works maximize accuracy under a latency budget. These works evaluate accuracy offline, one image at a time. However, real-time vision applications like autonomous driving operate in streaming settings, where ground truth changes between inference start and finish. This results in a significant accuracy drop. Therefore, a recent work proposed to maximize accuracy in streaming settings on average. In this paper, we propose to maximize streaming accuracy for every environment context. We posit that scenario difficulty influences the initial (offline) accuracy difference, while obstacle displacement in the scene affects the subsequent accuracy degradation. Our method, Octopus, uses these scenario properties to select configurations that maximize streaming accuracy at test time. Our method improves tracking performance (S-MOTA) by 7.4% over the conventional static approach. Further, performance improvement using our method comes in addition to, and not instead of, advances in offline accuracy.

==> Makefile <==
LATEX := pdflatex

all: paper.pdf

BIB := $(shell find . -name '*.bib')
FIGS := $(shell find figures/ -name '*.pdf')
TIKZ := $(shell find figures/ -name '*.tikz')
TEX := $(shell find . -name '*.tex')
EXTS = *.aux *.backup *.blg *.log *.out *.lof *.loa *.lot *.toc *.bbl *.bak \
       *.texshop *.dvi *.fdb_latexmk *.fls *.ent *.run.xml *.run.xml *.brf

paper.pdf: ${TEX}  ${TIKZ} ${BIB} ${FIGS}
	latexmk -pdf -bibtex paper.tex

push:
	scp paper.pdf ionel@login.eecs.berkeley.edu:public_html/pub/drafts/2022-policy-eccv.pdf

clean:
	latexmk -C
	rm -f paper.pdf
	rm -f ${EXTS}


==> evaluation-ablations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Evaluation Ablations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablations}
\label{ss:eval-ablations}

\begin{table}[tb]
  \scriptsize
  \centering
  \caption{\small \textbf{Comparing configuration ranking approaches}}
  \input{tables/LAT_AR-regression-baseline-ablations.tex}
  \label{t:class-vs-regression}
\end{table}

We conduct an ablation study of the experimental setup and the design choices.

\myparagraph{Baseline subtraction}
As a variance reduction technique, we consider regressing over the relative
score improvement from $h^{global}$ instead of absolute scores as described in
\ref{ss:policy-regression}.
%
Thus, we avoid dedicating model capacity to learn environment ``difficulty''
properties, which apply to all configurations in a manner that does not change
their score order.
%
As this distinction is not relevant for predicting configuration order, it only
introduces noise on the ranking downstream task~\cite{yogatama2014efficient}.
% %
% The latter factor depends on the environment's "perception difficulty".
% %
% Subtracting the global static configuration score decouples the latter factor
% and allows the model to focus on the change in configuration ranking, which is
% sufficient for determining the candidate \params{}. The performance of
% $H^{global}$ deviates on different scenarios indicative. The goal is to focus
% on modeling how score would differ from the global static configuration,
% instead of wasting model capacity on predicting the absolute score (which
% requires additional reasoning about the "difficulty" of the environment).
% learning to predict the \tmota{} score decreases the variance, making
% prediction easier.
Accordingly, in \Cref{t:class-vs-regression}, we observe a $0.3$ point increase
in \tmota{} score on the Waymo dataset when baseline subtraction is ablated.


We find that ranking via classification performs slightly worse than
with regression, and also that joint optimization of \params{} performs better
than independent optimization. These results
and analysis are in~\cref{app:eval-ablations-B}.

==> evaluation-runtime-analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Evaluation Runtime Analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Runtime Analysis of the \system{} Policy}
\label{ss:eval-policy-runtime}
The \system{} policy runs in parallel with the perception pipeline in order to
avoid delaying frame processing on the critical path.
% 
To avoid decision staleness, the \system{} policy must act on the previous
$\tau=1$ second step in a timely manner. Therefore, both policy decision and
actuation must execute quickly.

%
While the \system{} policy requires running inference on all of the $18$
configurations using Random Forest regression, we found our policy to be
sufficiently fast as its runtime is at most $6$ms on an Intel Xeon 8124M CPU.
%
Moreover, the policy is capable of actuating \param{} changes quickly.
%
During inference only the model weights and forward pass activations are stored
in GPU memory, allowing all the models to be pre-loaded simultaneously on a
single $32$GB GPU.
%
The policy also applies atomic changes to the tracking maximum age threshold,
allowing quick behavior change at runtime.


==> tables/LAT_AR-regression-baseline-ablations.tex <==
{
\begin{tabular}{@{}l|cccccc@{}}
    \toprule
    \textbf{Method}                     & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
    Regression w/o baseline subtraction & 27.6                          & 72.5                          & 31405                         & 610617                        & 8982                                            \\
    Regression w/ baseline subtraction  & 27.9                          & 72.3                          & 31489                         & 608870                        & 8966                                            \\ \bottomrule
    %Streaming Perception~\cite{streaming-perception} &       & 32.7          & \textbf{67.5} & 4184          & 161219          & 2420          \\
\end{tabular}
}


==> tables/argo-full.tex <==
{%\color{red}
% \setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}l|ccccc@{}}
    \toprule
    \textbf{Method}                         & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
    Global best                             & 55.5                          & 78.9                          & 9225                          & 51224                         & 1408 \\ \midrule
    Optimal                                 & 63.4                          & 76.8                          & 7357                          & 43142                         & 709  \\
    Optimal from the prev. segment          & 57.5                          & 76.8                          & 10024                         & 47917                         & 904  \\ \midrule
    \textbf{\system{}} with: & & & & &       \\
    Ground truth from current segment       & 58.7                          & 77.7                          & 8575                          & 48092                         & 1098 \\
    Ground truth from prev. segment         & 57.9	                    & 78.3                          & 8678                          & 48498                         & 1170 \\
    \textbf{Prediction from prev. segment } & \textbf{56.9}                 & \textbf{78.2}                 & \textbf{9376}                 & \textbf{49148}                & \textbf{1056} \\ \bottomrule
\end{tabular}
%Optimal \params{} on entire dataset \mota{} 40.2
}

% {
% \color{red}
% \begin{tabular}{@{}l|cccccc@{}}
%     \toprule
%     \textbf{Method}                                                & \textbf{\tmota{}} $\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
%     Optimal from 1 step in the past                                & 28.1                         & 71.4                        & 37211                       & 594927                      & 8192                                          \\ \midrule
%     Global best \params{}                                          & 27.2                         & 74.1                        & 21491                       & 620755                      & 11545                                         \\
%     \system{} with ground-truth Past Prediction ($\Delta \tau=1$s) & 28.4                         & 73.2                        & 30643                       & 601493                      & 9270                                          \\
%     \system{} with close-loop Past Prediction ($\Delta \tau=1$s)   & 28.0                         & 73.2                        & 29545                       & 605051                      & 9638                                          \\
%     \bottomrule
%     %Optimal \params{} past-1-step (4s)      &           &       &       &           &      \\
%     %Optimal \params{} past-1-step (1s)      &           &       &       &           &      \\ \bottomrule
%     %Global best \params{}                  & 34.0      & 65.1  & 5072  & 156492    & 2006 \\
% \end{tabular}
% }


==> tables/classification-ablations.tex <==
{
\begin{tabular}{@{}l|cccccc@{}}
    \toprule
    \textbf{Method}                         & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
    Classification (independent)            & 28.6                          & 73.1                          & 31668                         & 604054                        & 9463                                            \\
    Classification (joint)                  & 28.7                          & 73.0                          & 33975                         & 602491                        & 8916                                            \\
    Regression w/ baseline subtraction      & 28.9                          & 72.7                          & 31402                         & 598121                        & 9270                                            \\ \bottomrule
\end{tabular}
}


==> tables/classification-regression.tex <==
{
\begin{tabular}{@{}l|cccccc@{}}
\toprule
\textbf{Method}                      & \textbf{\tmota{}}$\uparrow{}$  & \textbf{\tmotp{}}$\uparrow{}$   & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
Classification (independent)            & 28.6 & 73.1 & 31668 & 604054 & 9463 \\
Classification (joint)                  & 28.7 & 73.0 & 33975 & 602491 & 8916 \\
Regression     w/o baseline subtraction & 28.7 & 72.8 & 32082 & 599085 & 9221 \\
Regression w/ baseline subtraction      &28.9  & 72.7 &	31402 &	598121 & 9270 \\ \bottomrule
%Streaming Perception~\cite{streaming-perception} &       & 32.7          & \textbf{67.5} & 4184          & 161219          & 2420          \\
\end{tabular}
}


==> tables/metaparameter-importance.tex <==
{
\setlength\tabcolsep{1.25pt}
\begin{tabular}{l|ccccc}
\toprule
\textbf{\Param{}} & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
Global best                & 27.2                        & 74.1                        & 21491                       & 620755                      & 11545    
\\
Detection-model	&	28.6 &	72.9 &	25692 &	605142 &	11749 \\
% D-Conf	    &	32.8&	\textbf{67.8}&	\textbf{3940}&	161586&  2301 \\
% D-Sched-Pol	&	32.8&	67.4&	4190&	161223&  2417 \\
% T-Min-Iou	&	32.7&	67.7&	4212&	161249&  2420 \\
Tracking-max-age	&27.8 &	73.7 &	28940 &	610219 &	8492 \\
   Both                     & 28.9                        & 72.7                        & 31402                       & 598121                      & 9270      
\\
% T-Reset-Freq&		32.7	&67.5&	4188&  161225&  2420 \\
\bottomrule

\end{tabular}

}


==> tables/optimization-gap.tex <==
\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}l|l|ccccc}
    \toprule
    \textbf{Method} & \textbf{Dataset} & \textbf{\mota{}}$\uparrow{}$  & \textbf{\motp{}}$\uparrow{}$  & \textbf{FP}$\downarrow{}$     & \textbf{FN}$\downarrow{}$     & \textbf{ID\textsubscript{sw}}$\downarrow{}$     \\ \midrule
    Global best     & Waymo            & 35.7                          & 78.7                          & 21364                         & 557480                        & 11370                                           \\
    Optimal         & Waymo            & 38.5                          & 77.9                          & 15787                         & 549702                        & 8694                                            \\
    Global best     & Argoverse        & 64.6                          & 83.1                          & 5554                          & 42303                         & 1271                                            \\
    Optimal         & Argoverse        & 72.7                          & 81.5                          & 5395                          & 32254                         & 739                                             \\ \bottomrule
    \toprule
    \textbf{Method} & \textbf{Dataset} & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
    Global best     & Waymo            & 27.2                          & 74.1                          & 21491                         & 620755                        & 11545                                           \\
    Optimal         & Waymo            & 32.1                          & 71.0                          & 28572                         & 582225                        & 7091                                            \\
    Global best     & Argoverse        & 55.5                          & 78.9                          & 9225                          & 51224                         & 1408                                            \\
    Optimal         & Argoverse        & 63.4                          & 76.8                          & 7357                          & 43142                         & 709                                             \\ \bottomrule
\end{tabular}

%% \begin{tabular}{@{}l|ccccc}
%%     \toprule
%%     \textbf{Method} & \textbf{\mota{}}$\uparrow{}$   & \textbf{\motp{}}$\uparrow{}$   & \textbf{FP}$\downarrow{}$   & \textbf{FN}$\downarrow{}$   & \textbf{ID\textsubscript{sw}}$\downarrow{}$   \\ \midrule
%%     Global best     & 35.7                        & 78.7                        & 21364                       & 557480                      & 11370                                         \\
%%     Optimal         & 38.5                        & 77.9                        & 15787                       & 549702                      & 8694                                          \\ \bottomrule
%%     \toprule
%%     \textbf{Method} & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
%%     Global best     & 27.2                        & 74.1                        & 21491                       & 620755                      & 11545                                         \\
%%     Optimal         & 32.1                        & 71.0                        & 28572                       & 582225                      & 7091                                          \\ \bottomrule
%% \end{tabular}


==> tables/regression-baseline-ablations.tex <==
{
\begin{tabular}{@{}l|cccccc@{}}
    \toprule
    \textbf{Method}                     & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
    Regression w/o baseline subtraction & 28.7                          & 72.8                          & 32082                         & 599085                        & 9221                                            \\
    Regression w/ baseline subtraction  & 28.9                          & 72.7                          & 31402                         & 598121                        & 9270                                            \\ \bottomrule
    %Streaming Perception~\cite{streaming-perception} &       & 32.7          & \textbf{67.5} & 4184          & 161219          & 2420          \\
\end{tabular}
}


==> tables/waymo-full.tex <==
{
% \setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}l|ccccc@{}}
    \toprule
    \textbf{Method}                         & \textbf{\tmota{}}$\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
    Global best                             & 27.2                        & 74.1                        & 21491                       & 620755                      & 11545                                         \\ \midrule
    Optimal                                 & 32.1                        & 71.0                        & 28572                       & 582225                      & 7091                                          \\
    Optimal from the prev. segment          & 28.1                        & 71.4                        & 37211                       & 594927                      & 8192                                          \\ \midrule
    \textbf{\system{}} with: & & & & & \\
    Ground truth from current segment       & 28.9                        & 72.7                        & 31402                       & 598121                      & 9270                                          \\
    Ground truth from prev. segment         & 28.4                        & 73.2                        & 30643                       & 601493                      & 9270                                          \\
    \textbf{Prediction from prev. segment}  & \textbf{28.0}               & \textbf{73.2}               & \textbf{29545}              & \textbf{605051}             & \textbf{9638}                                 \\ \bottomrule
\end{tabular}
%Optimal \params{} on entire dataset \mota{} 40.2
}

% {
% \color{red}
% \begin{tabular}{@{}l|cccccc@{}}
%     \toprule
%     \textbf{Method}                                                & \textbf{\tmota{}} $\uparrow{}$ & \textbf{\tmotp{}}$\uparrow{}$ & \textbf{\tfn{}}$\downarrow{}$ & \textbf{\tfp{}}$\downarrow{}$ & \textbf{\tid{}\textsubscript{sw}}$\downarrow{}$ \\ \midrule
%     Optimal from 1 step in the past                                & 28.1                         & 71.4                        & 37211                       & 594927                      & 8192                                          \\ \midrule
%     Global best \params{}                                          & 27.2                         & 74.1                        & 21491                       & 620755                      & 11545                                         \\
%     \system{} with ground-truth Past Prediction ($\Delta \tau=1$s) & 28.4                         & 73.2                        & 30643                       & 601493                      & 9270                                          \\
%     \system{} with close-loop Past Prediction ($\Delta \tau=1$s)   & 28.0                         & 73.2                        & 29545                       & 605051                      & 9638                                          \\
%     \bottomrule
%     %Optimal \params{} past-1-step (4s)      &           &       &       &           &      \\
%     %Optimal \params{} past-1-step (1s)      &           &       &       &           &      \\ \bottomrule
%     %Global best \params{}                  & 34.0      & 65.1  & 5072  & 156492    & 2006 \\
% \end{tabular}
% }

